Bipartite Graph Matching Algorithms for Clean-Clean Entity Resolution: An Empirical Evaluation

Entity Resolution (ER) is the task of finding records that refer to the same real-world entities. A common scenario is when entities across two clean sources need to be resolved, which we refer to as Clean-Clean ER. In this paper, we perform an extensive empirical evaluation of 8 bipartite graph matching algorithms that take in as input a bipartite similarity graph and provide as output a set of matched entities. We consider a wide range of matching algorithms, including algorithms that have not previously been applied to ER, or have been evaluated only in other ER settings. We assess the relative performance of the algorithms with respect to accuracy and time efficiency over 10 established, real datasets, from which we extract >700 different similarity graphs. Our results provide insights into the relative performance of these algorithms and guidelines for choosing the best one, depending on the data at hand.

==> tables/bahRunTime.tex <==
\begin{table}[t]\centering
 \setlength{\tabcolsep}{3pt}
    \caption{The average run-time (in seconds) of \textsf{BAH} per dataset and type of edge weights.}
    \vspace{-10pt}
    {\small
	\begin{tabular}{ | l | r | r | r | r | r | r | r | r | r | r |}
		\cline{2-11}
		\multicolumn{1}{c|}{}&
		\multicolumn{1}{c|}{$\mathbf{D_1}$} &
		\multicolumn{1}{c|}{$\mathbf{D_2}$} &
		\multicolumn{1}{c|}{$\mathbf{D_3}$} &
		\multicolumn{1}{c|}{$\mathbf{D_4}$} &
		\multicolumn{1}{c|}{$\mathbf{D_5}$} &
		\multicolumn{1}{c|}{$\mathbf{D_6}$} &
		\multicolumn{1}{c|}{$\mathbf{D_7}$} &
		\multicolumn{1}{c|}{$\mathbf{D_8}$} &
		\multicolumn{1}{c|}{$\mathbf{D_9}$} &
		\multicolumn{1}{c|}{$\mathbf{D_{10}}$} \\
		\hline
        \hline
        SBSY & 2$\pm$.0 & 1$\pm$.0 & 2$\pm$.1 & 2$\pm$.0 & 4$\pm$.8 & 3$\pm$.2 & 3$\pm$.3 & 124$\pm$.6 & 148$\pm$2 & 127$\pm$2 \\
        SASY & 2$\pm$.1 & 1$\pm$.0 & 2$\pm$.4 & 2$\pm$.3 & 3$\pm$.4 & 3$\pm$.4 & 4$\pm$.4 & 123$\pm$.4 & 145$\pm$2 & 128$\pm$2 \\
        SBSE & 2$\pm$.0 & 1$\pm$.0 & 2$\pm$.0 & 2$\pm$.1 & 3$\pm$.2 & 3$\pm$.2 & 3$\pm$.1 & 124$\pm$.3 & 148$\pm$3 & 129$\pm$1 \\
        SASE & 2$\pm$.1 & 1$\pm$.0 & 2$\pm$.0 & 2$\pm$.0 & 3$\pm$.0 & 3$\pm$.2 & 3$\pm$.2 & - & 149$\pm$3 & -\\
        \hline
	\end{tabular}
	\vspace{-10pt}
}
	\label{tb:runTime}
\end{table}

==> tables/d1Threshold.tex <==
\begin{table}[t]\centering
 \setlength{\tabcolsep}{2.5pt}
    \caption{The average similarity threshold and its standard deviation per dataset and type of input over $D_1$.}
    \vspace{-10pt}
    {\small
	\begin{tabular}{ | l | r | r | r | r | r | r | r | r | }
		\cline{2-9}
		\multicolumn{1}{c|}{}&
		\multicolumn{1}{c|}{\textbf{CNC}} &
		\multicolumn{1}{c|}{\textbf{RSR}} &
		\multicolumn{1}{c|}{\textbf{RCA}} &
		\multicolumn{1}{c|}{\textbf{BAH}} &
		\multicolumn{1}{c|}{\textbf{BMC}} &
		\multicolumn{1}{c|}{\textbf{EXC}} &
		\multicolumn{1}{c|}{\textbf{KRC}} &
		\multicolumn{1}{c|}{\textbf{UMC}} \\
		\hline
        \hline
        SYSB & .81$\pm$.15 & .85$\pm$.12 & .75$\pm$.14 & .83$\pm$.13 & .76$\pm$.14 & .69$\pm$.21 & .72$\pm$.17 & .71$\pm$.17 \\
        SASY & .60$\pm$.24 & .67$\pm$.20 & .64$\pm$.21 & .62$\pm$.23 & .64$\pm$.21 & .58$\pm$.21 & .60$\pm$.21 & .63$\pm$.22 \\
        SBSE & .70$\pm$.33 & .79$\pm$.23 & .79$\pm$.23 & .69$\pm$.34 & .77$\pm$.25 & .71$\pm$.25 & .74$\pm$.25 & .77$\pm$.26\\
        SASE & .80$\pm$.21 & .87$\pm$.11 & .80$\pm$.21 & .87$\pm$.11 & .80$\pm$.21 & .80$\pm$.21 & .80$\pm$.21 & .80$\pm$.21\\
        \hline
	\end{tabular}
	\vspace{-10pt}
}
	\label{tb:runTime}
\end{table}
